Learning Over Dirty Data with Minimal Repairs

Missing data often exists in real-world datasets, requiring significant time and effort for data repair to learn accurate models. In this paper, we show that imputing all missing values is not always necessary to achieve an accurate ML model. We introduce concepts of minimal and almost minimal repair, which are subsets of missing data items in training data whose imputation delivers accurate and reasonably accurate models, respectively. Imputing these subsets can significantly reduce the time, computational resources, and manual effort required for learning. We show that finding these subsets is NP-hard for some popular models and propose efficient approximation algorithms for wide range of models. Our extensive experiments indicate that our proposed algorithms can substantially reduce the time and effort required to learn on incomplete datasets.

==> minimalForLR.tex <==
\section{Minimal Repair for Linear Regression}
\label{sec:minimalLR}
The minimal repair for linear regression is the smallest set of features that is necessary to repair.
\begin{definition}\label{definition:minimalImputationLR}
Given the training set $(\mathbf{X}, \mathbf{y})$, a set of incomplete features in $\mathbf{X}$, denoted as $\mathbf{S}_{MR}(\mathbf{X}, \mathbf{y})$,
is a minimal repair for $(\mathbf{X}, \mathbf{y})$ for linear regression if we have: 1) a certain model exists upon imputing all missing values in the $\mathbf{S}_{MR}(\mathbf{X}, \mathbf{y})$, and 2) there is no set $\mathbf{S}$ satisfying condition (1) and $|\mathbf{S}| < |\mathbf{S}_{MR}|$.
\end{definition}

Similarly to Definition~\ref{definition:minimalImputation}, the existence of certain models in Definition~\ref{definition:minimalImputationLR} is orthogonal to the accuracy of imputation to $\mathbf{S}_{MR}$.
In linear regression, the optimal linear regression model $\mathbf{w}^*$ consists of the set of linear coefficients for feature vectors.
A feature $\mathbf{z}_i$ is considered relevant if the corresponding linear coefficient in the optimal model $w_i^*$ is not zero, and it is irrelevant if $w_i^*$ equals zero.
Intuitively, an incomplete feature needs to be repaired if it is relevant (i.e., it plays a role in the optimal model) and does not need to be repaired if it is irrelevant.
However, traditional statistical tools, such as the chi-square test, require complete distributions for each feature to assess correlations, which is challenging in the presence of missing values.
The minimal repair may not be unique.

\begin{theorem}\label{theorem:LRminImputeNotUnique}
There is a training set with multiple minimal repairs for linear regression.
In addition, if all the features in all the repairs of the training set $(\mathbf{X}, \mathbf{y})$ are linearly independent, the minimal repair for linear regression over $(\mathbf{X}, \mathbf{y})$ is unique.
\end{theorem}

The following theorem establishes that finding minimal repair for linear regression is intractable.
\begin{theorem}\label{theorem:LRNPhard}
Given a training set $(\mathbf{X},\mathbf{y})$ with incomplete features, finding the minimal repair for linear regression over $(\mathbf{X},\mathbf{y})$ is NP-hard.
\end{theorem}
To find minimal repair efficiently, we first propose an equivalent problem in Theorem \ref{theorem:linearregressionequivalent}, based on a variant of the well-known sparse linear regression problem \cite{bruckstein2009sparse}.

\begin{lemma}\label{theorem:linearregressionequivalent}
    Finding the minimal repair for linear regression on training set $(\mathbf{X}, \mathbf{y})$ is equivalent to:
\begin{align}
    \begin{array}{ll}
    \mathop{\min}\limits_{\mathbf{w}\in \mathcal{W}} T_{MF(\mathbf{X})}(\mathbf{w}) \\
    \text{subject to} \quad \mathbf{w} = \mathop{\arg\min}||\mathbf{X}^r\mathbf{w}-\mathbf{y}||^2_2, \forall \mathbf{X}^r \in \mathbf{X}^R
    \end{array}
\end{align}

where $T_{MF(\mathbf{X})}(\mathbf{w})$ is the number of non-zero linear coefficient in $\mathbf{w}$ whose corresponding feature is incomplete, i.e., $T_{MF(\mathbf{X})}(\mathbf{w}) = |\{\mathbf{z}_i \in MF(\mathbf{X})| w_i != 0\}|$
\end{lemma}

The distinction between our problem and sparse linear regression lies in their objectives: sparse linear regression seeks to minimize the number of non-zero coefficients across all features, whereas we focus on minimizing the number of non-zero coefficients only among incomplete features.
Orthogonal Matching Pursuit (OMP) provides an efficient approximation to solve the sparse linear regression problem \cite{wang2012generalized}.
This greedy algorithm begins with an empty solution set and initializes the regression residual to the label vector.
In each iteration, the algorithm selects the feature most relevant to the current residual (with largest dot product), adds it to the solution set, retrains a linear regression model, and updates the residual accordingly.
It stops when the regression residue is sufficiently small.

We propose a variant of OMP, as outlined in the appendix, to find minimal repair for linear regression.
Our algorithm has two major differences compared to the conventional OMP.
First, we include all complete features in the regression at the initialization, ensuring that we minimize the number of non-zero coefficients only among incomplete features.
Secondly, we define our stopping condition by the maximum relevance (cosine similarity) between the feature and the label being smaller than or equal to a user-defined threshold, instead of relying on a near-zero regression residue.
This approach enables our algorithm to work with general datasets without requiring the assumption of an underdetermined linear system, which is typically necessary in conventional OMP.

The time complexity of the algorithm is \(\mathcal{O}(T_{train} \cdot |MF(\mathbf{z})|)\), making it significantly more efficient than the baseline algorithm, which trains models on all repairs individually and has a time complexity of \(\mathcal{O}(T_{train} \cdot |\mathbf{X}^R|)\).
If we use gradient descent, our algorithm has a time complexity of \(\mathcal{O}(n \cdot d^3)\), where \(n\) is the number of training samples and \(d\) is the number of features.
In cases where \(n < d^2\), the time complexity is reduced to \(\mathcal{O}(n \cdot d^2 + n^2 \cdot d)\) under certain conditions by applying incremental learning techniques based on the Sherman-Morrison formula, as outlined in the appendix.
The following theorem characterizes the approximation rate of our algorithm.

\begin{theorem}\label{theorem:LRapproximatingrate}
    The first $k$ incomplete features added to $S_{MR}$ in our algorithm for training set $(\mathbf{X}, \mathbf{y})$ belong to a minimal repair of $(\mathbf{X}, \mathbf{y})$ with a probability of at least $1 - 1/n$, provided that: 1) $\mu < 1/(2k - 1)$, 2) the missing values in the dataset follow independent zero-mean normal distributions ($\mathcal{N}(0,\sigma^{2}_{ij})$),
    and 3) all linear coefficients ($w_i, \mathbf{z}_i \in MF(\mathbf{X})$) for incomplete features satisfy:
\begin{equation}
    |w_i| \geq \frac{2\sum_{x_{ij} = null}\sigma_{ij}\sqrt{n + 2\sqrt{n\log n}}}{1-(2k - 1)\mu}
\end{equation}

 where $\mu$ is the mutual incoherence defined by $\mu$ $=$ $\mathop{\max}\limits_{i \neq j} |\mathbf{z_i}^T\mathbf{z_j}|$.
\end{theorem}

==> supp_archived.tex <==
% \section*{\textcolor{red}{TODO}}
% 1. experimental-tables and charts, 2. replace all example with sample, replace all minimal imputation to minimal repair, 3. explain dataset with more details and also the evaluation metrics for linear regression and SVM, 4. Explain in some scenarios MR or AMR don't save (covered in Limitations section but might need some changes), 5. Hyperparameter tuning results with explanation, 6. Link to codebase, 7. Related work



% \section*{Limitations}

% While our work demonstrates both theoretical and practical advantages in learning over incomplete data, we acknowledge two limitations:

% \paragraph{Model Class and Convexity Assumptions.}
% Our proposed minimal repair (MR) algorithms are developed for support vector machines (SVM) and linear regression, while the almost minimal repair (AMR) framework is applicable to a broader class of statistical machine learning models. However, for AMR, we currently provide provable error bounds and efficient approximations only for models with convex loss functions. This stems from our reliance on Step 1 (ST1) in Section~5.1, where we solve a convex optimization problem to find an approximately optimal model $w_k^{\approx}$. Extending AMR to models with non-convex loss functions remains an open challenge due to the difficulty of verifying approximate optimality in such settings. Importantly, this limitation reflects the well-known hardness of non-convex optimization itself—since one cannot generally find globally optimal models for non-convex losses, it is also difficult to guarantee that a repaired model is close to a global optimum.

% \paragraph{Trade-off Between Computation and Imputation Time.}
% As seen in our experiments, the time required to compute MR or AMR can exceed or roughly match the time needed to fully impute the dataset when simple imputation methods (e.g., mean or KNN) are used. This suggests that MR and AMR may not be the preferred choice in scenarios where users already opt for inexpensive imputation strategies. However, for more complex, resource-intensive and often accurate imputation methods—such as diffusion-based models \cite{zheng2022diffusion}—we observe substantial time savings by using MR or AMR to reduce the number of imputations. In practice, users may choose to apply MR or AMR when planning to use high-cost imputation models, and directly pursue full imputation when using simpler methods.


\subsection{Approximating AMR for Deep Neural Networks}

Computing AMR for Deep Neural Networks (DNNs) is challenging as minimizing the suboptimality gap requires global minima for every repair. Recall that an ACM $\mathbf{w}^{\approx}$ satisfies:
\begin{equation}\label{equation:ACM_DNN}
\sup_{\mathbf{X}^r \in \mathbf{X}^R} \left( L(\mathbf{w}^{\approx}, \mathbf{X}^r, \mathbf{y}) - \min_{\mathbf{w} \in \mathcal{W}} L(\mathbf{w}, \mathbf{X}^r, \mathbf{y}) \right) \le e.
\end{equation}
Since flexible DNNs can memorize random data with near-zero loss \cite{zhang2016understanding, cooper2018loss}, we assume $\min_{\mathbf{w} \in \mathcal{W}} L(\mathbf{w}, \mathbf{X}^r, \mathbf{y}) \approx 0$. Thus, checking for an ACM simplifies to ensuring the worst-case loss is bounded.

To make this feasible, we check the condition sample-wise. We verify if the average difference between maximal and minimal repair losses satisfies the threshold $e$:
\begin{equation}\label{equation:ACMcheckdecomposeToSample}
\frac{1}{n} \sum_{\mathbf{x}_i \in MVX} \left( \max_{\mathbf{x}_i^r \in \mathbf{x}_i^R} L(f(\mathbf{x}_i^{r}, \mathbf{w}^{\approx}), y_i) - \min_{\mathbf{x}_i^r \in \mathbf{x}_i^R} L(f(\mathbf{x}_i^{r}, \mathbf{w}^{\approx}), y_i) \right) \leq e
\end{equation}
For networks with monotonic activations (e.g., ReLU), extrema occur at missing value boundaries (edge repairs), significantly reducing cost.

When the ACM condition is violated, AMR is the smallest subset restoring it. Intuitively, we impute samples contributing most to the loss difference in Eq. \ref{equation:ACMcheckdecomposeToSample}. Since this ranking is model-dependent, Algorithm \ref{alg:DNNAMR} collaboratively learns the DNN and identifies AMR via SGD.

\begin{algorithm}[!htbp]
\caption{Approximating AMR for Neural Networks}\label{alg:DNNAMR}
\begin{algorithmic}
\STATE $S_{AMR} \gets [\quad]$
\STATE $\mathbf{X}^{curr} \gets \text{random repair of } \mathbf{X}$; $\mathbf{w}^{curr} \gets \text{random initialization}$
\STATE $maxL, minL, samplesTopK \gets checkACM(\mathbf{w}^{curr}, \mathbf{X}^{curr})$
\WHILE{$maxL - minL > e$}
    \IF{$maxL > e$ \textbf{AND} $minL \leq e$}
        \STATE $\mathbf{X}^{curr} \gets impute(\mathbf{X}^{curr}, samplesTopK)$
        \STATE $S_{AMR} \gets S_{AMR}.add(samplesTopK)$
    \ENDIF
    \STATE $\mathbf{w}^{curr} \gets SGDEpoch(\mathbf{w}^{curr}, \mathbf{X}^{curr})$
    \STATE Update $maxL, minL, samplesTopK$
\ENDWHILE
\STATE \textbf{return} $S_{AMR}$
\end{algorithmic}
\end{algorithm}

The algorithm iteratively identifies $k$ samples to restore the ACM condition. Crucially, we only impute when the model is ``approximately optimal'' for some repairs ($minL \le e < maxL$). If both losses exceed $e$, we prioritize training ($SGDEpoch$) to ensure selection reflects true sample importance. $S_{AMR}$ is the union of imputed samples.









